CauDR: A Causality-inspired Domain Generalization Framework for Fundus-based Diabetic Retinopathy Grading

Diabetic retinopathy (DR) is the most common diabetic complication, which usually leads to retinal damage, vision loss, and even blindness. A computer-aided DR grading system has a significant impact on helping ophthalmologists with rapid screening and diagnosis. Recent advances in fundus photography have precipitated the development of novel retinal imaging cameras and their subsequent implementation in clinical practice. However, most deep learning-based algorithms for DR grading demonstrate limited generalization across domains. This inferior performance stems from variance in imaging protocols and devices inducing domain shifts. We posit that declining model performance between domains arises from learning spurious correlations in the data. Incorporating do-operations from causality analysis into model architectures may mitigate this issue and improve generalizability. Specifically, a novel universal structural causal model (SCM) was proposed to analyze spurious correlations in fundus imaging. Building on this, a causality-inspired diabetic retinopathy grading framework named CauDR was developed to eliminate spurious correlations and achieve more generalizable DR diagnostics. Furthermore, existing datasets were reorganized into 4DR benchmark for DG scenario. Results demonstrate the effectiveness and the state-of-the-art (SOTA) performance of CauDR.

==> experiments.tex <==
\section{Experiments}\label{sec:experiments}
Our study was implemented on a single NVIDIA RTX 3080 GPU and the official checkpoint of ViT-H SAM model was chosen to test the best performance of SAM on zero-shot medical image segmentation. After conducting tests across multiple medical imaging modalities, we observed that the segmentation outcomes were not consistently satisfactory among those modalities.



\subsection{Medical Image Segmentation Datasets}

Nine datasets (summarized in Table \ref{ALLDATA}), including Skin Lesion Analysis Toward Melanoma Detection \cite{codella2019skin,tschandl2018ham10000skin}, Drishiti-GS \cite{sivaswamy2015comprehensiveDrishti-GS}, RIM-ONE-r3 \cite{fumero2011rim}, REFUGE \cite{orlando2020refuge}, AMOS \cite{ji2022amos}, MICCAI 2017 Robotic Instrument Segmentation \cite{allan20192017robodata}, Chest X-ray \cite{candemir2013lungxray,jaeger2013automaticXRay}, Rat Colon \cite{park2017broadbandoct} and AROI \cite{melinvsvcak2021annotatedAROI} were used to examine the performance of SAM on medical image segmentation, covering a wide range of medical imaging modalities, such as OCT, MRI, and CT, as well as a diverse range of organs, including eyes, colon, spleen, kidney, gallbladder, esophagus, liver, and stomach.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table*}[]
% \centering
% \caption{\textcolor{red}{let's give more details of each dataset, e.g., how many data we used for testing, the year of publication}}
% \label{tab:dataset_details}
% % \scalebox{0.6}{
% \begin{tabular}{@{}ccc@{}}
% \toprule
% Dataset                                        & Modality       & Details          \\ \midrule
% Skin Lesion Analysis Toward Melanoma Detection~\cite{codella2019skin,tschandl2018ham10000skin} & Dermoscope     & Skin             \\
% Drishiti-GS~\cite{sivaswamy2015comprehensiveDrishti-GS} RIM-ONE-r3~\cite{fumero2011rim} REFUGE~\cite{orlando2020refuge} DRIVE~\cite{staal2004ridgeDRIVE}                                         & Fundus         & Eye              \\
% AMOS~\cite{ji2022amos}                                           & CT             & Abdominal organs \\
% AMOS~\cite{ji2022amos}                                           & MRI            & Abdominal organs \\
% MICCAI 2017 Robotic Instrument Segmentation~\cite{shvets2018automaticinstrument}    & Endoscope      & Tissue           \\
% Chest X-ray~\cite{jaeger2013automaticXRay,candemir2013lungxray}                                    & X-ray          & Chest            \\
% Rat Colon~\cite{park2017broadbandoct}                                      & Endoscopic OCT & Colon            \\
% AROI~\cite{melinvsvcak2021annotatedAROI}                                           & OCT            & Retinal          \\ \bottomrule
% \end{tabular}
% % }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\caption{Datasets Used for Examining the Zero-Shot Medical Image Segmentation Performance \mbox{of SAM}.}
\label{ALLDATA}
\begin{tabular}{@{}cccc@{}}
\toprule
Dataset                                        & Modality       & Details          & \multicolumn{1}{l}{Number of Test Samples} \\ \midrule
Skin Lesion Analysis Toward Melanoma Detection~\cite{codella2019skin,tschandl2018ham10000skin}  & Dermoscope     & Skin             & 259  \& 1000                                       \\
Drishiti-GS~\cite{sivaswamy2015comprehensiveDrishti-GS} RIM-ONE-r3~\cite{fumero2011rim} REFUGE~\cite{orlando2020refuge}                                           & Fundus         & Eye              & 51 \& 60 \& 160                                \\
AMOS~\cite{ji2022amos}                                           & CT             & Abdominal organs & 15361                                            \\
AMOS~\cite{ji2022amos}                                           & MRI            & Abdominal organs & 3176                                             \\
MICCAI 2017 Robotic Instrument Segmentation~\cite{allan20192017robodata}    & Endoscope      & Tissue           & 1200                                             \\
Chest X-ray~\cite{jaeger2013automaticXRay,candemir2013lungxray}                                     & X-ray          & Chest            & 704                                              \\
Rat Colon~\cite{park2017broadbandoct}                                      & Endoscopic OCT & Colon            & 130                                              \\
AROI~\cite{melinvsvcak2021annotatedAROI}                                           & SD-OCT            & Retina          & 113                                              \\ \bottomrule
\end{tabular}
\end{table*}

\subsection{Evaluation Metrics}
To assess the zero-shot segmentation capability of SAM on medical images, two quantitative metrics were employed: Dice similarity coefficient and Intersection over Union (IoU). The Dice coefficient measures the overlap between two sets of data and ranges from 0 (no overlap) to 1 (perfect overlap). Similarly, IoU computes the ratio of the intersection over the union of two sets and ranges from 0 to 1. Both metrics were then averaged across multiple samples to obtain an overall measure of the segmentation accuracy. Specifically, the Dice coefficient and IoU were calculated as

\begin{equation}
Dice = \dfrac{2 |Y \cap \hat{Y}|}{|Y| + |\hat{Y}|}
\end{equation}

\begin{equation}
IoU = \dfrac{|Y \cap \hat{Y}|}{|Y| + |\hat{Y}| - |Y \cap \hat{Y}|}
\end{equation}
where Y refers to the ground truth mask and \^{Y} denotes the predicted mask of SAM based on the prompt (i.e., the centroid of the ground truth mask). Dice and IoU are both the gold standards for evaluating the overlap of the ground truth and the predicted regions in image segmentation tasks. However, IoU is more suitable for evaluating the worst-case scenarios, which could provide a more comprehensive evaluation on the medical image segmentation. As some current methods use either one of these two evaluation metrics or both to report results, we use both Dice and IoU in our work to enable direct comparison.




\subsection{Results}

This section presents the results of zero-shot medical segmentation of SAM on eight different imaging modalities, as well as preliminary results of retinal vessel segmentation by fine-tuning SAM.


\begin{figure*}[!t]
\centerline{\includegraphics[width=\textwidth]{figures/good-sample.pdf}}
\caption{Successful segmentation examples of SAM. Eight distinct modalities labeled with (\textbf{A}--\textbf{H}) are included, corresponding to dermoscope, fundus, CT, MRI, RGB endoscope, X-ray, endoscopic OCT, and ophthalmic OCT. Each set of images comprises four images, containing two pairs of SAM segmentation versus corresponding ground truth (GT).}
\label{fig:good-samples}
\end{figure*}

\begin{figure*}[!t]
\centerline{\includegraphics[width=\textwidth]{figures/bad-sample.pdf}}
\caption{Failure segmentation examples of SAM. Eight distinct modalities labeled with (\textbf{A}--\textbf{H}) correspond to dermoscope, fundus, CT, MRI, RGB endoscope, X-ray, endoscopic OCT, and ophthalmic OCT. Each set of images consists of two paired SAM segmentation and ground truth (GT).}
\label{fig:bad-samples}
\end{figure*}


% \subsection{TODO}

% \begin{itemize}
%     \item \textcolor{red}{Create result table for each dataset (5 tables)}
%     \item \textcolor{red}{a figure showing good segmentation results, 4 columns, 2 examples per dataset (5 rows), using the following order for the column: sam/gt/sam/gt}
%     \item \textcolor{red}{a figure showing bad segmentation results, like above}

%     \item \textcolor{red}{a figure showing sam segmentation results that seem better than gt?? this one is optional, and we can just report one sample per dataset, or even without reporting for some datasets.}

% \end{itemize}





% \begin{enumerate}
\subsubsection{Dermoscopic Images}
Skin lesion analysis dataset is sourced from the challenge hosted by the International Skin Imaging Collaboration (ISIC) \cite{codella2019skin,tschandl2018ham10000skin}. Note that images captured by dermatoscopes with professional lighting and better magnification always present accurate details and precise contours. However, melanoma appears heterogeneously on different states of skin or diseases. Table \ref{skin} summarizes the results for comparison. From the bottom two rows of Table \ref{skin}, it is evident that for the same task, there is a significant difference in the final results due to the difference in the number of tested samples. We hypothesize that this discrepancy may be attributed to the randomness from the small number of samples. Therefore, the results from testing with larger number of samples may be more reliable. SAM (1000) refers to the performance of the model assessed on the official complete testing dataset. Additionally, as shown in Table \ref{skin}, the results of SAM are not competitive compared to existing methods. Specifically, SAM (259) denotes the outcome obtained by utilizing ten percent of randomly selected instances from the whole dataset as a testing subset, which facilitates a straightforward comparison with existing methods as using roughly ten percent of data has been a common practice in prior works. Figure \ref{fig:good-samples}A shows two samples that SAM perfectly segmented. As shown in Figure \ref{fig:good-samples}A, SAM is able to accurately segment the target when the anomalous regions are positioned at the center and exhibit a distinct morphology.



Figure \ref{fig:bad-samples}A shows two failure cases. When the target lesion locates in the erythematosus or scars, the segmentation often fails due to the similarity of features between the target and the adjacent parts or the absence of clear boundaries (or in another word, the lesion is less obtrusive or apparent).


% The quantities of both also correspond to the first row shown in Table~\ref{ALLDATA} at the same time. 
% \textcolor{red}{see my comments about in quantitative ... in review mode}




% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison with SOTA Methods on the Skin Lesion Analysis Toward Melanoma Detection Dataset.}
\label{skin}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccc@{}}
\toprule
Method      & Dice            & IoU             \\ \midrule
 U-Net~\cite{ronneberger2015unet}     & 0.8550          & 0.7850          \\
 UNet++~\cite{zhou2018unet++}     & 0.8090          & 0.7290        \\
 CaraNet~\cite{lou2022caranet}    & 0.8700          & 0.782          \\
 PraNet~\cite{fan2020pranet}     & 0.8750          & 0.7870          \\
 TransUNet~\cite{chen2021transunet}     & 0.8800          & 0.8090          \\ TransFuse~\cite{zhang2021transfuse}     & 0.9010          & 0.840          \\
 Double-UNet~\cite{jha2020doubleu}     & 0.8962          & 0.8212          \\
 Polyp-PVT~\cite{dong2021polyp}     & 0.8962          & 0.8212          \\
 DuAT~\cite{tang2022duat}     & 0.9230          & 0.8670          \\
 Polar Res-U-Net++(SOTA)~\cite{benvcevic2021skinsota} & \textbf{0.9253} & \textbf{0.8743} \\
\bottomrule
SAM (259 samples, common practice)     & 0.6636          & 0.5566          \\

 SAM (1000 samples, official test set)    & 0.7306          & 0.6169          \\
\bottomrule
\end{tabular}%
% }
\end{table}



\subsubsection{Fundus Images}
Retinal fundus images are considered as the primary modality in ophthalmic diagnosis. Specifically, optic cup (OC) and optic disc (OD) segmentation from the fundus image is the essential part. DoFE \cite{wang2020dofe} is a benchmark for OC and OD segmentation that comprises three different fundus image datasets. Due to the small size of available fundus image datasets, we amalgamated the data used in DoFE to evaluate the performance of SAM. 
% Such an approach serves to alleviate the possibility of incidental experimental results. In the follow-up process, 
Apart from an overall evaluation, we also explored and examined the domain generalization of SAM based on the same domain partitions as DoFE.

% In this benchmark, we utilized a few prompts for OC and OD segmentation to explore SAM's zero-shot performance on enclosed regions \textcolor{red}{what is difference between enclosed and closed mentioned earlier? not annular??} \textcolor{blue}{not pretty sure about difference between those, enclosed should be distinct from the branching structures as vessels of fundus image} of fundus images. 
Note that OC constitutes a whitish, cup-shaped area situated at the center of the OD, which can be approximated as two concentric circles of different radius. Specifically, the fundus images were first cropped to better observe the region of interest (ROI). The positions of two prompts exhibit a high degree of proximity, occasionally coinciding with each other.
% \textcolor{blue}{In terms of choosing appropriate prompts, other choices could be considered, e.g., bounding boxes, as prompts of proximal location are difficult to accurately guide the segmentation of OC and OD.} 
Thus, accurately segmenting between OC and OD is not easy when receiving similar prompts. This partly causes zero-shot SAM to only have half of the accuracy of current SOTAs. We hypothesize that manually prompting SAM (i.e., oracle) may lead to a better accuracy though the zero-shot mode of SAM may still lag behind SOTA by a noticeable margin.

% It is conjectured that the difference in segmentation results between these two types is due to the fact that the area of OC is smaller than OD, and OC is the higher contrast part of the ROI, which may be more common in the training set of SAM from natural scenes.

We also investigated the performance of SAM on cross-domain scenarios following the setting in DoFE \cite{wang2020dofe}. The imbalanced performance observed in Table \ref{fundus} demonstrates that the domain generalization (DG) problem also exists in SAM. SAM achieves the best and worst mean performance on domain 1 and domain 4.
% The major differences between domains result from different imaging devices or scan protocols. These appearance discrepancies would affect the generalization ability of the model, which caused DG issues. 
By inspecting fundus images from four domains, we found that the degree of contrast between OC/OD and background is proportional to the final performance. However, this proportional relationship cannot be observed in DG-optimized algorithms in Table \ref{fundus}. This comparison reveals that SAM mainly focuses on superficial features (image contrast) instead of high-level semantics when zero-shot segmenting OC/OD in fundus images. Figures~\ref{fig:good-samples}B and~\ref{fig:bad-samples}B show some successful and failed fundus segmentation samples, respectively.
% , which would cause poor generalization and worthless clinic values in practice. 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \begin{table}[]
% \centering
% \caption{}
% \label{undefined}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% Method  & \multicolumn{3}{c}{Dice}          & \multicolumn{3}{c}{IoU}           \\ \midrule
%         & Mean   & OC              & OD     & Mean   & OC              & OD     \\ \cmidrule(l){2-7} 
% Domain 1 & 0.5637 & 0.5710 & 0.5563 & 0.4120 & 0.4227 & 0.4012 \\
% Domain 2 & 0.4267 & 0.5200 & 0.3333 & 0.2993 & 0.3760 & 0.2227 \\
% Domain 3 & 0.4993 & 0.5830 & 0.4157 & 0.3616 & 0.4437 & 0.2794 \\
% Domain 4 & 0.3827 & 0.3598 & 0.4056 & 0.2680 & 0.2465 & 0.2896 \\
% All & 0.4609 & \textbf{0.5116} & 0.4102 & 0.3296 & \textbf{0.3752} & 0.2841 \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


% \begin{table*}[]
% \centering
% \caption{Comparison with the State-of-the-Art Methods on Fundus Datasets evaluated by the Dice Similarity Coefficient}
% \label{undefined}
% \scalebox{1}{
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% \multirow{3}{*}{Method} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2} & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & Mean \\ \cmidrule(l){2-10} 
%       & \multicolumn{9}{c}{Dice}                                                                \\ \cmidrule(l){2-10} 
%       & OC     & OD     & OC     & OD     & OC     & OD     & OC     & OD     & Total           \\ \midrule
% U-Net & 0.7703 & 0.9496 & 0.7821 & 0.8969 & 0.8028 & 0.8933 & 0.8474 & 0.9009 & 0.8554          \\ \midrule
% Mixup & 0.7332 & 0.9297 & 0.7112 & 0.8678 & 0.8216 & 0.9042 & 0.8623 & 0.9076 & 0.8423          \\
% DST   & 0.7563 & 0.9220 & 0.8080 & 0.9077 & 0.8432 & 0.9402 & 0.8624 & 0.9066 & 0.8683          \\
% JiGen & 0.8081 & 0.9503 & 0.7946 & 0.9047 & 0.8265 & 0.9194 & 0.8430 & 0.9106 & 0.8697          \\
% DoFE  & 0.8359 & 0.9559 & 0.8000 & 0.9837 & 0.8666 & 0.9198 & 0.8704 & 0.9332 & \textbf{0.8844} \\
% SAM   & 0.5710 & 0.5563 & 0.5200 & 0.3333 & 0.5830 & 0.4157 & 0.3598 & 0.4056 & 0.4609          \\ \bottomrule
% \end{tabular}}
% \end{table*}


\begin{table*}[]
\centering
% \caption{}
\caption{Comparison with SOTA Methods on Fundus Datasets Evaluated using the Dice Similarity Coefficient.}
\label{fundus}
\scalebox{1}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2} & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & Mean \\ \cmidrule(l){2-10} 
      & OC     & OD     & OC     & OD     & OC     & OD     & OC     & OD     & Total           \\ \midrule
U-Net~\cite{ronneberger2015unet} & 0.7703 & 0.9496 & 0.7821 & 0.8969 & 0.8028 & 0.8933 & 0.8474 & 0.9009 & 0.8554          \\
Mixup~\cite{zhang2017mixup} & 0.7332 & 0.9297 & 0.7112 & 0.8678 & 0.8216 & 0.9042 & 0.8623 & 0.9076 & 0.8423          \\
DST~\cite{zhang2019DST}   & 0.7563 & 0.9220 & \textbf{0.8080} & 0.9077 & 0.8432 & \textbf{0.9402} & 0.8624 & 0.9066 & 0.8683          \\
JiGen~\cite{carlucci2019jigen} & 0.8081 & 0.9503 & 0.7946 & 0.9047 & 0.8265 & 0.9194 & 0.8430 & 0.9106 & 0.8697          \\
DoFE~\cite{wang2020dofe}  & \textbf{0.8359} & \textbf{0.9559} & 0.8000 & \textbf{0.9837} & \textbf{0.8666} & 0.9198 & \textbf{0.8704} & \textbf{0.9332} & \textbf{0.8844} \\ \bottomrule
SAM   & 0.5710 & 0.5563 & 0.5200 & 0.3333 & 0.5830 & 0.4157 & 0.3598 & 0.4056 & 0.4609          \\ \bottomrule
\end{tabular}%
}
\end{table*}


\subsubsection{Endoscopic OCT}
For endoscopic OCT, the OCT Rat Colon dataset \cite{park2017broadbandoct} was used, which was captured by an 800-nm ultrahigh-resolution endoscopic SD-OCT system \cite{yuan2022vivo}. The colonic wall is composed of three distinct layers for segmentation, namely colonic mucosa (CM), submucosa (SM), and muscularis externa (ME). A tenth of dataset was randomly sampled in our experiment to evaluate the performance of SAM. Images in this dataset do not contain much color information and complex structures, which is supposed to be easy for segmentation. Nevertheless, the zero-shot segmentation performance of SAM on endoscopic OCT is far inferior to models specifically designed for medical images as shown in Table \ref{rat oct}. Figures \ref{fig:good-samples}G and \ref{fig:bad-samples}G show some segmentation samples of SAM. It can be observed that compared to successful examples of other datasets, the successful examples of endoscopic OCT are actually not perfect, while the failure cases are indeed unsatisfactory.

\begin{table}[]
\centering
\caption{Comparison with SOTA Methods on the OCT Rat Colon Dataset.}
\label{rat oct}
\begin{tabular}{@{}cccc@{}}
\toprule
Method                   & Class     & Dice            & IoU             \\ \midrule
TransUNet~\cite{chen2021transunet}                     & All & \textbf{0.9265} & \textbf{-} \\ 
LiDeOCTNet~\cite{abaxi2023lideoctnet}                     & All & 0.9198 & \textbf{-} \\ \midrule
\multirow{4}{*}{SAM} & Colonic Mucosa  & 0.3491          & 0.2350          \\
                         & Submucosa  & 0.2477          & 0.1485          \\
                         & Muscularis Externa  & 0.2399          & 0.1466          \\
                         & All & 0.2789          & 0.1767          \\ \bottomrule 
\end{tabular}
\end{table}
    
\subsubsection{Ophthalmic OCT} 
Annotated Retinal OCT Images Database (AROI) \cite{melinvsvcak2021aroi} contains 1136 annotated B-scans and associated raw high-resolution images from 24 patients with age-related macular degeneration (AMD). An ophthalmologist annotated three retinal layers and three retinal fluids in each B-scan. The official annotations on B-scan are utilized to classify eight layered structures, including the inner plexiform layer and inner nuclear layer (IPL/INL), as well as regions above internal limiting membrane (ILM) and under bruch's membrane (BM). Pigment epithelial detachment (PED), subretinal fluid and subretinal hyperreflective material (SRF), and intraretinal fluid (IRF) are also involved for segmentation. We did not take the top layer (above ILM) into consideration (i.e., not tested), because it is not a part of internal structure of retina.
% The credibility of predictive accuracy is not entirely dependable, whereby regions that are easily segmented exhibit pronounced precision while non-coherent and small areas yield unreliable segmentation results. 
% As a consequence, when calculating overall accuracy, each partitioned segment is weighted equally, which limits the ability of this measure to accurately assess the predictive capacity of SAM for the eight distinct segments. 

As shown in Table \ref{oct}, the segmentation results for under BM are much higher than other classes, which is also confirmed by the qualitative samples shown in Figure \ref{fig:good-samples}H. This indicates that SAM can accurately segment the structures of clear boundaries and large continuous areas. However, the zero-shot segmentation performance of SAM is extremely unsatisfactory for small holes and elongated layered structures of irregular boundaries (such as RPE-BM), as shown in Figure \ref{fig:bad-samples}H.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{Zero-Shot Segmentation Results of SAM for Different Classes from the AROI Dataset.}
\label{oct}
\begin{tabular}{@{}ccc@{}}
\toprule
Class & Dice            & IoU             \\ \midrule
ILM-IPL/INL   & 0.2378          & 0.1527          \\
IPL/INL-RPE   & 0.4499          & 0.3153          \\
RPE-BM   & 0.0688          & 0.0368          \\
under BM   & \textbf{0.8704} & \textbf{0.7806} \\
PED   & 0.1083          & 0.0673          \\
SRF   & 0.1084          & 0.0656          \\
IRF   & 0.0923          & 0.0548          \\ \midrule
Average  & 0.3237          & 0.2506          \\ \bottomrule
\end{tabular}
\end{table}



\subsubsection{CT}  
AMOS \cite{ji2022amos} contains both CT and MRI modalities for abdominal multi-organ segmentation tasks. The entire dataset introduces 500 CT and 100 MRI volume data from 15 organs in abdominal cavity. During pre-processing, we set the CT window range to [$-$991, 362] HU and 15361 slices from the dataset were generated using this standard. Since the corresponding ground truth in the test set has not been released, we used the validation set which contains segmentation labels. Fifteen organs were segmented, including spleen, right kidney, left kidney, gallbladder, esophagus, liver, stomach, aorta, inferior vena cava, pancreas, right adrenal gland, left adrenal gland, duodenum, bladder, prostate and uterus. The above described are also applied to MRI and the experimental results of CT are therefore presented and discussed along with those of MRI in the next section for clarity. 

% \begin{table}[]
% \centering
% \caption{}
% \label{undefined}
% \begin{tabular}{@{}ccc@{}}
% \toprule
% Class   & Mean Dice       & Mean IoU        \\ \midrule
% \#1     & 0.1121          & 0.0612          \\
% \#2     & 0.2687          & 0.2202          \\
% \#3     & 0.3288          & 0.2737          \\
% \#4     & 0.1198          & 0.0916          \\
% \#5     & 0.1442          & 0.1056          \\
% \#6     & 0.3056          & 0.2044          \\
% \#7     & 0.2428          & 0.1587          \\
% \#8     & \textbf{0.3332} & \textbf{0.2748} \\
% \#9     & 0.1429          & 0.1051          \\
% \#10    & 0.1547          & 0.1052          \\
% \#11    & 0.0768          & 0.0628          \\
% \#12    & 0.1114          & 0.0852          \\
% \#13    & 0.1823          & 0.1275          \\
% \#14    & 0.1137          & 0.0622          \\
% \#15    & 0.0404          & 0.0211          \\ \midrule
% Total & 0.2154          & 0.1609          \\ \bottomrule
% \end{tabular}
% \end{table}
\begin{table}[]
\centering
\caption{Zero-Shot Segmentation Results of SAM on Different CT Organ Classes in AMOS Dataset.}
\label{sam on CT}
\begin{tabular}{@{}ccc@{}}
\toprule
Class   & Dice       & IoU        \\ \midrule
\#1     & 0.1616          & 0.1026          \\
\#2     & 0.2723          & 0.2211          \\
\#3     & \textbf{0.3465}          & \textbf{0.2856}          \\
\#4     & 0.0943          & 0.0630          \\
\#5     & 0.1023          & 0.0724          \\
\#6     & 0.3188          & 0.2097          \\
\#7     & 0.2624          & 0.1812          \\
\#8     & 0.2946          & 0.2310 \\
\#9     & 0.1555          & 0.1188          \\
\#10    & 0.1375          & 0.0930          \\
\#11    & 0.0287          & 0.0202          \\
\#12    & 0.0585          & 0.0454          \\
\#13    & 0.1831          & 0.1284          \\
\#14    & 0.1292          & 0.0752          \\
\#15    & 0.0653          & 0.0360          \\ \midrule
Average & 0.2105          & 0.1548          \\ \bottomrule
\end{tabular}
\end{table}


\subsubsection{MRI} 
 The pre-processing method of MRI data is congruent with the one used for CT data mentioned in the preceding section. A total of 3176 images originating from the validation set were obtained and selected for our case study. As the datasets of two modalities are derived from the same dataset and the 3D data were pre-processed in a same way, the average Dice scores of the two modalities are close as shown in Table~\ref{sam on CT} and Table~\ref{sam on MRI}, although the variations exist across individual class segmentation tasks. As shown in Figure \ref{fig:good-samples}C, D, SAM can accurately segment two-dimensional organs in CT and MRI images. The successful segmentation manifests the precise localization and clear demarcation, and a striking resemblance to the actual organ structures in terms of visual appearance. However, the failure cases shown in \mbox{Figure \ref{fig:bad-samples}C, D} are often from the segmentation of small organs, in which SAM exhibits a tendency to segment not only the target organ itself but also the neighboring tissues.
% \begin{table}[]
% \centering
% \caption{}
% \label{undefined}
% \begin{tabular}{@{}ccc@{}}
% \toprule
% Class   & Mean Dice & Mean IoU \\ \midrule
% \#1     & 0.4252    & 0.3195   \\
% \#2     & 0.5556    & 0.4781   \\
% \#3     & 0.4991    & 0.3981   \\
% \#4     & 0.0331    & 0.0172   \\
% \#5     & 0.0431    & 0.0246   \\
% \#6     & 0.5206    & 0.4203   \\
% \#7     & 0.1037    & 0.0556   \\
% \#8     & 0.3877    & 0.3177   \\
% \#9     & 0.1111    & 0.0816   \\
% \#10    & 0.1591    & 0.1069   \\
% \#11    & 0.0080    & 0.0040   \\
% \#12    & 0.1897    & 0.1500   \\
% \#13    & 0.1887    & 0.1341   \\ \midrule
% Total & 0.2271    & 0.1731   \\ \bottomrule
% \end{tabular}
% \end{table}
\begin{table}[]
\centering
\caption{Zero-Shot Segmentation Results of SAM on Different MRI Organ Classes in AMOS Dataset.}
\label{sam on MRI}
\begin{tabular}{@{}ccc@{}}
\toprule
Class   & Dice & IoU \\ \midrule
\#1     & 0.2571    & 0.1785   \\
\#2     & \textbf{0.4622}    & \textbf{0.3866}   \\
\#3     & 0.4434    & 0.3656   \\
\#4     & 0.1437    & 0.1026   \\
\#5     & 0.0352    & 0.0207   \\
\#6     & 0.4480    & 0.3311   \\
\#7     & 0.1475    & 0.0912   \\
\#8     & 0.2843    & 0.2285   \\
\#9     & 0.0691    & 0.0452   \\
\#10    & 0.1175    & 0.0754   \\
\#11    & 0.0054    & 0.0027   \\
\#12    & 0.0243    & 0.0177   \\
\#13    & 0.0989    & 0.0642   \\ \midrule
Average & 0.2264    & 0.1723   \\ \bottomrule
\end{tabular}
\end{table}


\subsubsection{X-Ray}    
 The dataset (704 labelled images) used for testing SAM on X-ray is compiled from the validation and training sets of \cite{candemir2013lungxray,jaeger2013automaticXRay}. As shown in Figure \ref{fig:good-samples}F, the segmentation performance demonstrated by SAM in successful cases is impressive and the segmentation results perfectly match with the ground truth. However, the failure cases shown in \mbox{Figure \ref{fig:bad-samples}F} reveal that the zero-shot chest X-ray segmentation of SAM is not always consistent. Table \ref{x-ray} shows the quantitative results of zero-shot X-ray image segmentation.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{Quantitative Results of Zero-Shot SAM on an X-ray Dataset.}
\label{x-ray}
\begin{tabular}{@{}ccc@{}}
\toprule
Method  & Dice   & IoU    \\ \midrule
SAM & 0.6509 & 0.5136 \\ \bottomrule
\end{tabular}
\end{table}





\subsubsection{Endoscopic Images}   
We further tested SAM on the MICCAI 2017 Robotic Instrument Segmentation dataset \cite{shvets2018automaticinstrument}, which contains 2040 stereo camera images acquired from a da Vinci Xi surgical system on three types of segmentation task (binary, parts and instruments segmentation). The images are essentially captured by RGB cameras. As a result, the segmentation outcomes shown in Figure \ref{fig:good-samples}E are impressive when appropriate prompts are given. As we place the prompt at the center of each individual object, a three-class segmentation of parts is the most suitable choice for testing in order to avoid any irregular connections and interference between different parts compared with binary segmentation and instrument segmentation. The performance of SAM was tested using data from the official testing set, and the results were compared against those provided in the official report. To better visualize, segmentation results of different categories have been plotted onto the same graph for comparison, which are shown in both Figures \ref{fig:good-samples}E and \ref{fig:bad-samples}E. {It should be noted that even though some examples exhibit visually satisfactory results, they are likely due to the predicted masks partially lying within other masks.} From a quantitative perspective as shown in Table \ref{medrobo}, SAM has already surpassed the segmentation performance of LinkNet-34 \cite{shvets2018automaticinstrument,chaurasia2017linknet} by only receiving prompts. However, it is still not comparable to the current SOTA and there is a 30\% relative gap between SAM and SOTA methods.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Comparison with SOTA Methods on the MICCAI 2017 Robotic Instrument Segmentation Dataset.}
\label{medrobo}
\begin{tabular}{@{}cccc@{}}
\toprule
Method                   & Class   & Dice            & IoU             \\ \midrule
UNet~\cite{ronneberger2015unet}                     & All    & 0.6075          & 0.4841          \\ 
TernausNet-16~\cite{shvets2018automaticinstrument}            & All    & \textbf{0.7597} & \textbf{0.6550} \\ 
TernausNet-11~\cite{shvets2018automaticinstrument}            & All    & 0.7425          & 0.6223          \\ 
LinkNet-34~\cite{shvets2018automaticinstrument}               & All    & 0.4126          & 0.3455          \\ \midrule
\multirow{4}{*}{SAM} & Clasper & 0.4296          & 0.3054          \\
                         & Wrist   & 0.5076          & 0.3674          \\
                         & Shaft   & 0.7189          & 0.5076          \\
                         & All    & 0.5512          & 0.4227          \\ \bottomrule
\end{tabular}
\end{table}


    
\subsubsection{Retinal Vessel in Fundus Images}
    
\begin{figure}[htbp] 
	
	\centering
	
	\includegraphics[width=\linewidth,scale=0.5]{figures/fail-sample.pdf}
	\caption{A failure sample of SAM on segmenting retinal vessels. The first row from left to right is: the initial input image, ground truth mask, and the input image superimposed with the ground truth mask. The second row from left to right shows three SAM segmented images with the score of 1.007, 0.993, and 0.673, respectively.}
	\label{fail-sample}
	
\end{figure}


\begin{figure}[htbp] 
	
	\centering
	
	\includegraphics[width=\linewidth,scale=0.5]{figures/finetune-sample2.pdf}
	\caption{Segmentation samples of SAM fine-tuned on retinal vessels. Each row from left to right is the initial input image, ground truth mask and prediction of fine-tuned SAM. The column from top to bottom shows retinal images from four different datasets.}
	\label{finetune-sample}
	
\end{figure}

We also used SAM to segment vessels in fundus images. However, the experiments revealed that zero-shot SAM is not able to accurately segment retinal blood vessels, despite the \textit{manual} provision of additional prompts focused on areas where visibility of vessels is pronounced. At the current stage, we conjectured that the segmentation of continuously branching structures, such as blood vessels in medical images and tree branches in nature images, presents a challenge for SAM. As shown in Figure \ref{fail-sample}, it is found that SAM encounters difficulties in accurately identifying vessels as distinct segmentable objects.
Therefore, we further conducted fine-tuning of SAM to examine its potential of improving segmentation results. To fine tune SAM (SAM ViT-B in this experiment), we utilized SAM adapter \cite{chen2023samadapter}, a task-specific fine-tuning method proposed for SAM. Specifically, 20 image-mask pairs were selected from the Digital Retinal Images for Vessel Extraction (DRIVE) dataset \cite{staal2004ridgeDRIVE} to fine-tune SAM's mask decoder. As the fine-tuning was fully supervised, there was no prompt provided and the ground truth masks were used to supervise the training. The entire fine-tuning process was trained with the AdamW \cite{loshchilov2017adamw} optimizer. The learning rate was set to {$2 \times 10^{-4}$} %MDPI: please change the terms into scientific notations, e.g., “8 × 10³”, not “8E3”.
with a total of 20 training epochs. The batch size was one with the input image size of 1024 $\times$ 1024 pixels. A total of four datasets were utilized for the quantitative assessment. Three of them are the official test sets from their respective datasets. The official training set from the STARE dataset \cite{hoover2000STARE} was also employed for testing as its own test set is lacking. As shown in Table \ref{quatitive result of fine-turn}, the fine-tuned SAM demonstrated substantial improvements in both the Dice and IoU metrics. Noticeably, the Dice scores increased by at least 200 percent relative to its zero-shot counterpart where vessels were segmented by manually providing the prompt. Furthermore, the improvements of IoU were even more pronounced. In addition, as illustrated in Figure \ref{finetune-sample}, the segmentation results of SAM after fine-tuning almost perfectly match with ground truth in some cases and only some tiny parts at the terminal ends of vessels are missing, demonstrating the potential of SAM for precise medical image segmentation after a domain-specific fine-tuning.    

\begin{table*}[]
\centering
\caption{Quantitative Results of Fine-tuned SAM on Retinal Vessel Segmentation Datasets.}
\label{quatitive result of fine-turn}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
Dataset  & Dice (Manual) & Dice (Fine-tuned) & Dice Relative Increase & IoU (Manual) & IoU (Fine-tuned) & IoU Relative Increase \\ \midrule
DRIVE~\cite{staal2004ridgeDRIVE}    & 0.2267       & 0.7733         & 241\%                  & 0.1281      & 0.6304        & 392\%                 \\
CHASEDB1~\cite{fraz2012CHASEDB1} & 0.1685       & 0.7118         & 322\%                  & 0.0921      & 0.5526        & 500\%                 \\
HRF~\cite{odstrcilik2013HRF}      & 0.1701       & 0.6776         & 298\%                  & 0.0931      & 0.5124        & 450\%                 \\
STARE~\cite{hoover2000STARE}    & 0.1902       & 0.7694         & 304\%                  & 0.1057      & 0.6252        & 491\%                 \\ \bottomrule
\end{tabular}}
\end{table*}

% \end{enumerate}
